Raw Image Reconstruction with Learned Compact Metadata

While raw images exhibit advantages over sRGB images (e.g., linearity and fine-grained quantization level), they are not widely used by common users due to the large storage requirements. Very recent works propose to compress raw images by designing the sampling masks in the raw image pixel space, leading to suboptimal image representations and redundant metadata. In this paper, we propose a novel framework to learn a compact representation in the latent space serving as the metadata in an end-to-end manner. Furthermore, we propose a novel sRGB-guided context model with improved entropy estimation strategies, which leads to better reconstruction quality, smaller size of metadata, and faster speed. We illustrate how the proposed raw image compression scheme can adaptively allocate more bits to image regions that are important from a global perspective. The experimental results show that the proposed method can achieve superior raw image reconstruction results using a smaller size of the metadata on both uncompressed sRGB images and JPEG images.

==> content/intro.tex <==
\section{Introduction}
As an unprocessed and uncompressed data format \wh{directly obtained from camera sensors}, raw images provide unique advantages for computer vision tasks in practice.
%
%For example, the noise distribution in raw space is easy to be modeled so that models trained on raw space have better denoising capacity~\cite{zhang2021rethinking, abdelhamed2019noise}. 
\wh{For example, it is easier to model the distribution of real image noise in raw space, which enables generalized deep real denoising networks~\cite{zhang2021rethinking, abdelhamed2019noise};}
%
%Benefited from the characteristic that the pixel values have a linear relationship with scene radiance, raw image also greatly contributes to the low-light image enhancement~\cite{wei2020physics}.
%
\wh{As the pixel values in raw images have a linear relationship with scene radiance, it owns the benefit to recover shadows and highlights without bringing in the grainy noise usually associated with high ISO settings, which greatly contributes to the low-light image enhancement~\cite{wei2020physics, huang2022towards}.}
%One of the largest benefits of RAW is the capactiy to recover shadows and highlights in post-processing without bringing in the grainy noise usually associated with high ISO settings. RAWs are very forgiving if you have severely underexposed or overexposed areas.
%
%Besides, raw image also provides more space for the corrections and artistic manipulation due to the more shades of colors.
\wh{Besides, with richer colors, the raw image offers more room for correction and artistic manipulation.}

\begin{figure}[t]
    \centering
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figure/intro_fig1.pdf}
    \caption{Previous SOTA methods sample in the raw space \cite{punnappurath2021spatially, nam2022learning}.}
     \end{subfigure}
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figure/intro_fig2.pdf}
    \caption{The proposed method samples in the latent space.}
     \end{subfigure}
    % \includegraphics[width=0.95\linewidth,height=0.5\linewidth]{figure/intro_fig.pdf}
    \caption{
    The comparison between the previous SOTA methods (in gray) and our proposed method (in blue).
    %
    Different from the previous work where the sampling strategy is hand-crafted or learned by a pre-defined sampling loss, we learn the sampling and reconstruction process in a unified end-to-end manner. 
    %
    In addition, the sampling of previous works is in the raw pixel space, which in fact still includes a large amount of spatial redundancy and precision redundancy.
    %
    Instead, we conduct sampling in the feature space, and more compact metadata is obtained for pixels in the feature space via the adaptive allocation. (The saved metadata is annotated in dashed box.)
    }
    \label{fig:intro}
    \vspace{-0.3cm}
\end{figure}

Despite of these merits, raw images are not widely adopted by common users \wh{due to} large file sizes. 
%
\wh{In addition, since raw images are unprocessed,}
%it requires additional time for raw images to do the post-processing before displaying, \wh{\textit{e.g.}}, demosaicing, and denoising.
additional post processing steps, \textit{e.g.}, demosaicing and denoising, are always needed before displaying them.
%
%Therefore, even if the raw images are saved, a copy \wh{in JPEG format} is usually saved.
For fast image rendering in practice, a copy of JPEG image is usually saved along with its raw data \cite{dng}.
%
To improve the storage efficiency, raw-image reconstruction problem attracts more and more attention, \textit{i.e.}, how to minimize the amount of metadata required for de-rendering sRGB images back to raw space.
%
Classic metadata-based raw image reconstruction methods model the workflow of image signal processing (ISP) pipeline and save \wh{the required parameters in ISP} as metadata \cite{nguyen2016raw}.
%
\wh{To further reduce the storage and computational complexity towards a lightweight and flexible reverse ISP reconstruction, very recent methods focus on sparse sampling of raw image pixels \cite{punnappurath2021spatially, nam2022learning}.}
%Recently, methods based on the sparse sampling of raw pixels \cite{punnappurath2021spatially, nam2022learning} are becoming mainstream due to the increasing complexity of the ISP.
% Need to be processed.
%\whc{Recently, methods based on the sparse sampling of raw pixels \cite{punnappurath2021spatially, nam2022learning} are becoming mainstream due to the increasing complexity of the ISP.}{The logic is not clear here. Why does the increasing complexity has an effect on sampling methods? Something is missing.}
%
Specifically, \wh{in~\cite{punnappurath2021spatially},} a uniform sampling strategy \wh{is proposed to combine} with \wh{an} interpolation algorithm \wh{that solves} systems of linear equations. 
%
\wh{The work in~\cite{nam2022learning} proposes a sampling network and approximates the reconstruction process by deep learning to further improve the sampling strategy}.


Though lots of progress has been made, existing sparse sampling based raw image reconstruction methods still face \wh{limitations} in terms of \wh{coding} efficiency and image reconstruction quality. 
%
\wh{Specifically, in the idea case, affected by global/local non-linear mapping and quantization loss, the information loss \yf{caused by the ISP} should be non-uniform as shown in Fig. \ref{fig:isp}.
%
More specially, the spatial sampling rate should be content adaptive. 
%
For example, in a flat region, less information is enough for guaranteeing the reconstruction quality while in the texture or edge regions, we get the opposite conclusion.}
%
\wh{However, in existing practices, even for the \wh{state-of-the-art} method~\cite{nam2022learning} where the sampling is enforced to be locally non-uniform, it is still almost uniform from the global perspective, which causes bit-rate redundancy and limits the reconstruction performance.}

To address the above issues, instead of adopting a pre-defined sampling strategy or sampling loss, \textit{e.g.}, super-pixel loss, we propose a novel end-to-end learned raw image \textit{joint sample-reconstruction framework} based on the encoded latent feature with the entropy constraint as shown in Fig. \ref{fig:intro}.
%
To further improve the rate-distortion performance, we propose an sRGB guided context model. % 
%
\wh{By introducing the sRGB images to guide the entropy coding of raw images, the context model becomes feasible and effective in raw image reconstruction, greatly \wh{increasing} the \wh{compression/decompression} speed while \wh{maintaining} comparable performance to commonly used \wh{auto-regressive} models~\cite{cheng2020learned, minnen2018joint}}.

\wh{Our contributions are summarized} as follows\wh{,}
\begin{enumerate}
    \item We propose the first end-to-end deep encoding framework for raw image reconstruction, by fully optimizing the use of stored metadata.
    % \item \wh{As far as we know, we are the first to incorporate end-to-end learned coding technologies into the raw image reconstruction framework by making full use of the metadata, including both hand-crafted and learned ones.}
    %
    \item A novel sRGB-guided context model is proposed by introducing two improved entropy estimation strategies, which leads to better reconstruction quality, smaller size of metadata, and faster speed.
    % \item \wh{Based on the proposed framework, we further propose improved entropy estimation strategies based on a novel sRGB-guided context model}
    %
    \item \wh{We evaluate our method over popular raw image datasets. The experimental results demonstrate that we can achieve better reconstruction quality with less metadata required comparing with SOTA methods.}
\end{enumerate}


